Recursive Estimation of Orientation Based on the Bingham Distribution

Directional estimation is a common problem in many tracking applications. Traditional filters such as the Kalman filter perform poorly because they fail to take the periodic nature of the problem into account. We present a recursive filter for directional data based on the Bingham distribution in two dimensions. The proposed filter can be applied to circular filtering problems with 180 degree symmetry, i.e., rotations by 180 degrees cannot be distinguished. It is easily implemented using standard numerical techniques and suitable for real-time applications. The presented approach is extensible to quaternions, which allow tracking arbitrary three-dimensional orientations. We evaluate our filter in a challenging scenario and compare it to a traditional Kalman filtering approach.

==> BibTeX-ISAS/ISASPubl_Keys.tex <==
\renewcommand{\refname}{\normalsize \Deutsch{Preprints}\English{Preprints} (6)}
\begin{bibunit}
  \nocite{
  	% From here 06/24/12
	arXiv12_Hekler,
	arXiv12_Hanebeck,
	arXiv12_Deisenroth,
	arXiv11_Kretz,
	arXiv11_Lyons,
	arXiv10_Perez}
  	% To here 06/24/12
  \putbib
\end{bibunit}

\renewcommand{\refname}{\normalsize \Deutsch{Artikel in Konferenzb\"anden}\English{Conference Papers} (218)}
\begin{bibunit}
  \nocite{
  	% From here 11/02/12
  	CDC12_Baum,
	CDC12_Chlebek,
	CDC12_Hekler,
	CDC12_Noack,
	CDC12_Reinhardt,
	IROS12_Faion,
	MFI12_Baum,
	MFI12_Reinhardt,
  	% To here 11/02/12  
  	% From here 06/24/12
	Fusion12_Baum,
	Fusion12_BaumWillett,
	Fusion12_Faion-CylinderTracking,
	Fusion12_Faion-RecursiveCalibration,
	Fusion12_Fischer,
	Fusion12_Gilitschenski,
	Fusion12_Hanebeck,
	Fusion12_Hekler,
	Fusion12_Noack,
	Fusion12_Packi,
	Fusion12_Reinhardt,
	Fusion12_Reinhardt-FastCI,
	ACC12_Hekler,
	ACC12_Lyons,
	SPIE12_FischerBaum,
	TRB12_Kretz,
	CDC11_Baum,
	CDC11_Hekler,
	ICCV11_Kretz,
	Humanoids11_Rybok,
	SDF11_Huber,
	IROS11_Baum,
	IROS11_Gehrig,
	IROS11_Perez,
	TGF11_Kretz,
	IFAC11_Huber,
	IFAC11_Noack,
	Fusion11_Baum-RHM,
	Fusion11_Baum-USF,
	Fusion11_Baum,
	Fusion11_Bogatyrenko,
	Fusion11_Krauthausen,
	Fusion11_Noack,
	Fusion11_Reinhardt,
	Fusion11_Ruoff,
	% Up tp here 06/24/12
 	ACC11_Bogatyrenko,
 	ACC11_Huber,
 	ACC11_Krauthausen,
 	ACC11_Noack,
	EWSN11_Schmid,
	CDC10_Hekler,
	IROS10_Beutler,
	IROS10_Bogatyrenko,
	IROS10_Packi,
	IROS10_Perez,
	IROS10_Krauthausen,
	SDF10_Baum,
	KI10_Krauthausen,
	IPIN10_Packi,
	VECIMS10_Baum,
	MFI10_Baum,
	MFI10_BaumRect,	
	MFI10_BaumGheta,
	MFI10_Beutler,
	MFI10_Bogatyrenko,
	MFI10_KrauthausenEberhardt,
	MFI10_Krauthausen,
	MFI10_LyonsHekler,
	MSC10_HeklerLyonsNoack,
	Fusion10_BaumKlumpp,
	Fusion10_BaumNoack,
	Fusion10_Beutler,
	Fusion10_DunauPacki,
	Fusion10_EberhardtKlumpp,
	Fusion10_Klumpp-SGMF,
	Fusion10_Klumpp,
	Fusion10_KrauthausenHuber,
	Fusion10_Noack,
	SUTC10_Lyons,
	ACC10_Eberhardt,
	ACC10_Krauthausen,
	PED10_Perez,
%	NIPS09_Deisenroth,
	ISSPIT09_Baum,
%	Deisenroth2009,
	CDC09_HanebeckHuber,
	IROS09_Bogatyrenko,
	SDF09_Baum,
	CCA09_RauhHanebeck,
	Fusion09_Baum,
	Fusion09_Beutler,
	Fusion09_Hoerst-SGMF,
	Fusion09_Huber,
	Fusion09_Klumpp-FusionND,
	Fusion09_Klumpp-Type2Dens,
	Fusion09_Krauthausen,
	Fusion09_Noack,
%	Fusion09_Schieferdecker,
	MSRL09_Deisenroth,
	ICINCO09_Perez,
	ICML09_Deisenroth,
	CASA09_Perez,
	ICASSP09_Beutler,
	MFI09_Beutler,
	ICASSP09_Beutler,
	MFI08_Hanebeck-LCD,
	MFI08_HuberBailey,
	MFI08_Klumpp-DiracFusion,
	MFI08_Klumpp-DiracTrees,
	MFI08_NaWang,
	MFI08_Sawo-Localization,
	MFI08_Schwarzenberg,
	MFI08_WangSzabo,
	MFI08_WeisselSchreiter,
	IFAC08_Huber,
	IFAC08_SawoBeutler,
	IFAC08_WeisselHuber,
	Fusion08_Huber-PGMR,
	Fusion08_Huber_PLSS,
	Fusion08_KlumppSawo-SGMF,
	Fusion08_Noack-ConvexSets,
	Fusion08_SawoKlumpp-SimParam,
	Fusion08_Wang,
	CDC07_HanebeckSchrempf,
	CDC07_WeisselHuber,
	IROS07_SchrempfAlbrecht,
	IROS07_WeisselHuber,
	SDF07_Huber,
	HCI07_Wang,
	Fusion07_HanselmannSchrempf,
	Fusion07_Huber,
	Fusion07_SawoHuber-ParamIdent,
	ACC07_Huber,
	ACC07_Schrempf-DiracMixt,
	ACC07_WeisselHuber,
	ECC07_DeisenrothWeissel,
	CARS07_Roberts,
	ICINCO07_Schrempf-DiracMixt,
	ICINCO07_WeisselHuber,
	IPSN07_Huber,
	ICRA07_Bader,
	WPNC07_Wang,
	CDC06_Brunn-Fourier,
	CDC06_Schrempf-DiracMixt,
	IROS06_Roessler,
	HCRS06_SchrempfSchmid,
	HCRS06_RoesslerSchrempf,
	CCA06_Sawo-ParameterizedGM,
	MFI06_Beutler,
	MFI06_Brunn-Fourier,
	MFI06_DeisenrothWeissel,
	MFI06_Huber,
	MFI06_Schrempf-CramerMises,
	MFI06_Wang,
	ICINCO06_Roessler,
	ICINCO06_SawoRoberts,
	Fusion06_Klumpp,
	Fusion06_Sawo-ParameterizedGMs,
	Fusion06_SchrempfHanselmann,
	ECC05_Rauh,
	INTETAIN05_Groenda,
	CSIT05_Weissel,
	ICINCO05_Hahn,
	ICINCO05_Roessler,
	ICINCO05_Schrempf-Intention,
	ROMAN05_SchrempfSchmid,
%	CCA05_Sawo,
	IROS05_Roessler,
	Fusion05_Roberts,
	Fusion05_Schrempf-MixtureReduction,
	IFAC05_Schrempf-HybridBN,
	ICRA05_Brunn-Splines,
	ICASSP05_Beutler,
	Sensors04_Beutler,
	CSIT04-Schrempf_HybridBN,
	SMC04_Roessler,
	MECHROB04_Roessler,
%	IPDPS04_Weissel,
	CDC03_Feiermann-ProgBayes,
	ECC03_Hanebeck,
	ECC03_Horn-SetBasedLocalization,
	SYSID03_Hanebeck,
	MFI03_Hanebeck,
	SPIE03_HanebeckBriechle-ProgBayes,
	SPIE03_Horn,
	SPIE03_Nitzsche,
	SPIE03_Rauh,
	HCRS02_Nitzsche,
%	DSP02_Roessler,
	ICRA02_Lorch,
	LOCELLUS02_Horn,
	ROMAN01_Nitzsche,
	ECC01_Hanebeck-SetTheoreticEst,
	ECC01_HanebeckHorn-BoundsRandomNoise,
	ECC01_HanebeckHorn-MixStochSetUncertainty,
	MFI01_Hanebeck-PseudoEllipsoids,
	MFI01_HanebeckBriechle-UnknownCorr,
	MFI01_HanebeckHorn-CovarianceBound,
	ACC01_Hanebeck,
	ACC01_HanebeckHorn-MixStochSetUncertainty,
	GMA01_Hanebeck,
	SPIE01_BriechleHanebeck_CrossCorr,
	SPIE01_HanebeckHorn-SLAM,
	RAAD00_Saldic,
	CDC99_Hanebeck,
	SMC99_Briechle-SLAM,
	SMC99_Hanebeck-MixStochSetUncert,
	IROS99_HanebeckSaldic-WheelSystem,
	IROS99_HanebeckHorn-StochSetUncert,
	ECC99_Hanebeck,
	ICRA99_Hanebeck,
	SPIE99_Hanebeck,
	ROMAN98_Schmidt,
	AMC98_Furtwaengler,
	ICRA98_Hanebeck,
	IARP97_Hanebeck,
	IROS97_Hanebeck,
	ISER97_Hanebeck,
	ICASSP96_Hanebeck,
	ICRA96_Hanebeck-SetBayes,
	ICRA96_HanebeckSchmidt-Angle,
	ICASAV95_Hanebeck,
	TELEMAN95_Maier,
	ICONIP94_Hanebeck,
	IROS94_Hanebeck,
	EUFIT94_Hanebeck,
	IFAC93_Hanebeck}
  \putbib
\end{bibunit}

\renewcommand{\refname}{\normalsize \Deutsch{Artikel in B\"uchern}\English{Papers in Books} (18)}
\begin{bibunit}
  \nocite{
	VMS10_Lyons,
	VMS10_Noack,
	VMS10_Kuwertz,
	LNEE_ICINCO08_WeisselHuber,
	LNEE_ICINCO08_Schrempf,
	LNEE_ICINCO07_SawoRoberts,
	IMS06_BrunnSawo,
	AMS05_RobertsSzabo,
	AMS03_Roessler,
	AMS00_Briechle,
	Robotik00_Hanebeck,
	AMS99_Briechle,
	AMS98_Furtwaengler,
	ISER98_Hanebeck,
	AMS96_Daxwanger,
	AMS95_Hanebeck,
	IRS95_Hanebeck,
	KI95_Hanebeck}
  \putbib
\end{bibunit}

\renewcommand{\refname}{\normalsize \Deutsch{Artikel in Zeitschriften}\English{Journal Papers} (20)}
\begin{bibunit}
  \nocite{
   	% From here 11/02/12
 	TAES_Baum,
	TRAC12_Deisenroth,  	
  	% SYSAES_Baum,
	% To here 11/02/12
	TM10_Noack,
	TM10_Kuwertz,
	IJCARS10_Bogatyrenko,
	ITM07_BrunnSawo,
	AT05_Briechle,
	AT05_Grigoras,
	PRE04_Nitzsche,
	RA04_Briechle,
	SPL03_Rauh,
	AT03_Nitzsche,
	DGON02_Horn,
	IF00_Hanebeck,
	AT00_Hanebeck,
	AUTO99_Hanebeck,
	JIRSTA98_Ettelt,
	CEP96_Hanebeck,
	FSS96_Hanebeck,
	AT93_Hanebeck}
  \putbib
\end{bibunit}

\renewcommand{\refname}{\normalsize \Deutsch{Sonderhefte, B\"ucher}\English{Special Issues, Books} (3)}
\begin{bibunit}
  \nocite{
    KI10_Hanebeck,
	AT05_Hanebeck,
	AMS99_Schmidt}
  \putbib
\end{bibunit}

\renewcommand{\refname}{\normalsize \Deutsch{Habilitation, Dissertation, Diplomarbeit, Studienarbeit}\English{Habilitation, Dissertation, Diploma Thesis, Student Research Project} (4)}
\begin{bibunit}
  \nocite{
	Habil02_Hanebeck,
	Diss97_Hanebeck,
	DA91_Hanebeck,
	SA89_Hanebeck}
  \putbib
\end{bibunit}

==> BibTeX-ISAS/ISAS_SADA_Keys.tex <==
\renewcommand{\refname}{\normalsize \Deutsch{Diplomarbeiten in Karlsruhe}\English{Supervised Diploma Theses in Karlsruhe}}
\begin{bibunit}
  \nocite{
	DA10_Berg,
	DA08_Hirsch,
	DA08_Gehrig,
	DA08_Moellers,
	DA08_Khairallah,
	DA07_Bluemel,
	DA07_Richter,
	DA07_Stiegeler,
	DA07_Schreiter,
	DA07_Krekeler,
	DA07_Meyer,
	DA07_Groene,
	DA07_Seth,
	DA07_Herdtweck,
	DA07_Hanselmann,
	DA07_Albrecht,
	DA07_Krieg,
	DA06_Kern,
	DA06_Beisler,
	DA06_Deisenroth,
	DA06_Klumpp,
	DA06_Huber,
	DA05_Hauth,
	DA05_Prokop,
	DA04_Schrempf,
	DA04_Hahn,
	DA03_Mayer,
	DA03_Misch}
  \putbib%[ISAS_SADA]
\end{bibunit}

\renewcommand{\refname}{\normalsize \Deutsch{Studienarbeiten in Karlsruhe}\English{Supervised Student Research Projects in Karlsruhe}}
\begin{bibunit}
  \nocite{
	SA10_Reinhardt,
	SA10_Petkov,
	SA08_Kuwertz,
	SA08_Hoerst,
	SA07_Reinbold,
	SA07_Noack,
	SA07_Packi,
	SA07_StefanMeyer,
	SA07_Ota,
	SA07_Zaschke,
	SA07_Stiegeler,
	SA07_Eberhardt,
	SA07_Hauth,
	SA06_Schieferdecker,
	SA06_Baer,
	SA06_Ek,
	SA06_Eberling,
	SA06_Winkler,
	SA06_Stoll,
	SA06_Mende,
	SA06_Hessel,
	SA06_Omid,
	SA06_Armstrong,
	SA06_Hanselmann,
	SA06_Herb,
	SA05_Juetting,
	SA05_Kern,
	SA05_JohannesMeyer,
% 	SA05_GerhardMeyer,	% existiert nicht: ist SA05_JohannesMeyer
	SA05_Krieg,
	SA05_Schamburek,
	SA04_Deisenroth,
	SA04_Lamprecht}
  \putbib%[ISAS_SADA]
\end{bibunit}

\renewcommand{\refname}{\normalsize \Deutsch{Studien--, Semester-- und Diplomarbeiten an der TU M\"unchen}\English{Supervised Student Research Projects and Diploma Theses at TU M\"unchen}}
\begin{bibunit}
  \nocite{
	DA02_Rauh,
	DA01_Riegel,
	DA01_Dabringhaus,
	DA01_Huber,
	SA00_Lohninger,
	SA00_Lohn,
	DA00_Molitor,
	DA99_Russ,
	SA99_Leclerc,
	DA97_Kroessler,
	SA97_Urli,
	DA96_Suess,
	DA95_Maier,
	DA94_Stegmeier,
	DA94_Richter,
	DA93_Berger,
	DA93_Grabl,
	DA93_Boegholm,
	SA93_Roul,
	SA93_Pelat,
	SA92_Faeustle}
  \putbib%[ISAS_SADA]
\end{bibunit}



